Precision Studies of QCD in the Low Energy Domain of the EIC

The manuscript focuses on the high impact science of the EIC with objective to identify a portion of the science program for QCD precision studies that requires or greatly benefits from high luminosity and low center-of-mass energies. The science topics include (1) Generalized Parton Distributions, 3D imagining and mechanical properties of the nucleon (2) mass and spin of the nucleon (3) Momentum dependence of the nucleon in semi-inclusive deep inelastic scattering (4) Exotic meson spectroscopy (5) Science highlights of nuclei (6) Precision studies of Lattice QCD in the EIC era (7) Science of far-forward particle detection (8) Radiative effects and corrections (9) Artificial Intelligence (10) EIC interaction regions for high impact science program with discovery potential. This paper documents the scientific basis for supporting such a program and helps to define the path toward the realization of the second EIC interaction region.

==> Additional.tex <==
\section{Additional text- not to be fully included }

{\color{blue} \underline{V.B.}:{\bf {\color{blue} Some alternate thoughts on the "mass" topic and on emergent mass. This is not meant as a
contribution to the text, but as a point of discussion. Mass of matter is not a fixed number but changes with temperature. These processes are being studied at RHIC by energy scans (changing temperature in the plasma). } It would be nice to have some discussion of this, maybe in an introduction. It may allow connecting studies of heavy ion collisions and of the EIC science.} }  \\

{\color {blue} V.B.: As scientist we not only want to understand the universe as it is, but also how it evolved from 
the Big Bang 
through various phase transitions to the present time. 
Just microseconds after it came into existence, the universe entered in a crossover period from the quark-gluon plasma 
phase to the hadron phase that was characterized by a cool down to the few-hundred MeV temperature range, 
accompanied by the emergence of hadron resonances, the occurrence of chiral symmetry breaking and the 
emergence of confinement and stable baryons. This is being studied in hot-LQCD simulations.The transition 
temperature appears to be near 155 MeV. These processes are currently 
being studied experimentally at RHIC in high-energy heavy ion collisions with the ongoing energy scan. The large gap  
between hot-LQCD and hadron resonance models that include known strange- charmed-states, show that many hadrons 
carrying strange and charm flavors are still 
to be found to solve part of the missing baryon pressure gap in Fig.\Ref{universe}. 
The EIC could play a very important role in their discovery, especially in the charmed quark sector.   \\
\begin{figure}[h] 
\hspace{-0.2cm}\includegraphics[width=0.34\columnwidth]{figures/universe_chronology.jpg}
\hspace{1.0cm}\includegraphics[width=0.40\columnwidth]{figures/strange-charm-pressure.png}
\caption{Chronology of the evolution of the universe (left). The crossover from the quark-gluon plasma 
phase to the hadron phase (right) takes place at about 1$\mu$sec, with the critical temperature near 155 MeV. 
Markers show Lattice calculations for strange and charm baryon/meson versus temperature from weekly 
interacting quarks at high temperatures to near bound quarks below 150 MeV. Lines indicate hadron gas 
model calculations with hadron states as tabulated in RPP20xx and hadrons from full quark model. 
Lines do not fit the hot-LQCD results, indicating significant amount of missing baryons pressure of 
strange and charm flavor. Similar but lower missing baryon pressure is observed for light-quark baryons.} 
\label{universe}
\end{figure}

\noindent How can we study the emergence of hadron rest masses at the EIC? 
It has been known for some time that the fundamental Higgs mechanism~\cite{Higgs} leads to masses of 
elementary quarks. 
However, in the light-quark sectors of u-quarks and d-quarks such as the nucleon and its excitation spectrum 
in the baryon sector, and light unflavored mesons such as the $\pi$, $\rho$ and their excitation  
in the meson sector, elementary quark masses $\rm m_q$ contribute only a few MeV to the hadrons rest mass $\rm M_h$, 
leaving much of $\rm M_h$ to be generated by the gluons and their dynamical interactions with the 
quarks and with other gluons to give rise to the quark's "constituent" mass $m_Q$ of several hundred MeV/c$^2$.  delete. xji}

{\color{red} XJI: this is a wrong picture for mass. There is
a mass scale $\Lambda_{QCD}$, quark kinetic energy will
generate large contribution to the mass, gluon has the standard energy contribution as $E^2 + B^2$}. {\color{green} VB: How do gluons factor into that picture? gluon has the standard energy contribution as $E^2 + B^2$ }\\

{\color{blue} The model of a "constituent" quark mass $\rm m^Q$ has been shown in light-cone relativistic quark model~\cite{Aznauryan} with 
running quark mass, and in continuum QCD related studies~\cite{Segovia}, not to be constant, but to depend on
the distance scale at which the proton's structure is probed, e.g. in elastic scattering and in resonance 
excitation processes at high photon virtuality. Virtual photons in the range $Q^2 > 50$GeV$^2$ will be 
required to begin seeing the transition effect of elementary quark interaction as is shown in Fig.~\ref{fig-x}.
With increasing photon virtuality the gluon cloud is increasingy penetrated and probes closer to the 
elementary mass. If expressed in reverse order, by probing the quarks at smaller $Q^2$, the quarks begin to 
get dressed increasingly with gluons leading to increasingly higher effective masses. In analogy to the evolution 
of the universe, or high-energy heavy ion collisions, it corresponds to the hadron mass emerging at lower temperature, 
or lower energy transfer. \\

The dynamics of the emerging hadron mass could be studied best in measurement in the valence 
quark regime and at elastic processes $ep \to ep$ and resonance transitions in $ep \to e\pi^+ n, eK^+\Lambda, ep \pi^+\pi^-$ and other reactions at high $Q^2$, focusing on the $x_B > 0.05 $ range. This requires highest luminosity at low CM energies. 
The kinematics at lowest CM energy is shown in shown in Fig.~\ref{EIC-kine1}. } \\


==> GPDs3D-old.tex <==

\section{Generalized parton distributions and precision spatial imaging}% (F.X. Girod, V. Burkert, X. Ji, C. Hyde, \underline {S. Liuti}, F. Sabati\'e)}
%
\label{sec:GPD}
\subsection{3D imaging of the nucleon: the new science of nuclear femtography}
\label{sec:IIIA}
The science of nuclear femtography probed in deeply virtual exclusive scattering (DVES) has revolutionized our approach to exploring the internal structure of the nucleon. 
%
We can now aspire to reconstruct spatial images of the nucleon's interior in terms of its quark and gluon constituents, while simultaneously unveiling the mechanisms that give origin to its spin and mass from a multitude of strongly interacting quark and gluon fields. 
%

Key objects to reconstruct 3D structure from data are the generalized parton distributions (GPDs) which are specific projections in longitudinal momentum and transverse coordinate space of the relativistic Wigner phase-space distributions. 
%GPDs bridge information between PDFs and FFs. 
Remarkably, their Mellin moments in $x$ are directly related to the matrix elements between proton states of the QCD energy-momentum tensor (EMT). GPDs, therefore, bring the EMT, which would, otherwise, only be probed through gravity, within experimental grasp through electromagnetic scattering.

The experiments currently planned at Jefferson Laboratory and other facilities worldwide as well as the new generation of experiments at the future EIC will provide a wealth of data which will be processed in order to image the 3D quark and gluon structure of the proton at the femtoscale. Data in a wide breath in $x_{Bj}$, $t$  and $Q^2$,  will be complemented by information from phenomenology and lattice QCD calculations to produce tomographic images of the deepest layers of  visible matter. 

The ambitious program of generating femtoscale images of the nucleon brings phenomenological analyses of data to a new level where expertise including theoretical and experimental physics, math and computer science intersect. First and foremost, each individual experiment can only add a small piece to the picture: 
%This is needed to separate out the GPDs by type (helicity structure) and flavor. 
%The complexity is such the ML methods will be necessary. 
harnessing and organizing information from experiments will require going beyond the standard data analysis methods and computational toolboxes by implementing state of the art Machine Learning techniques.
Furthermore, to increase the reach of this emergent field information from previous experiments will need to be folded into the analyses so as to provide a full coverage of the phase space needed to form realistic images. Theoretical guidance on the various aspects of GPDs and cross sections details will be crucial at every step. 

In Fig.~\ref{fig:E-H} we show one of the projected results for the 2-dimensional images of the CFF $\mathcal{E(\xi,\it t)}$ and $\mathcal{H(\xi,\it t)}$ Fourier transformed into impact parameter space $(b_x, b_y)$ \textcolor{magenta}{where is this from ??? SL}. The image was extracted from
simulated measurements of different polarization asymmetries and cross sections with the proton 
transversely polarized. Kinematic coverage is assumed for a 12 GeV electron beam and fixed target experiments in the valence quark region. At the EIC such images may be obtained at varies values of $\xi = 10^{-3} - 10^{-1}$ for high luminosity operation at medium cm energies $\sqrt{s} = 28 - 45$ GeV.   

{\bf I consider this figure a filler. Need reference. Insert gluon image. {\color{blue} I have inquired with FX about reference. I don't know that there is an image for gluon distribution.}} 
%%%%
\begin{figure}[htb!]
    \centering
    \includegraphics[width=0.8\columnwidth]{figures/GPD-E-polTarget.png}
    \caption{Images of the 2-dimensional distribution of $\cal{H} + \cal{E}$  in the valence region for a 
    spin-polarized proton with the polarization axis parallel to $b_x$ (left graph). The polarization causes small vertical 
    shifts. The right graph shows the effect of $\cal{E}$ with the effect of the polarization more 
    dramatically seen as clear spatial separation of electrical charges, i.e. u- and d-quarks in $b_y$ space, 
    generating a flavor-dipole. }
    \label{fig:E-H}
\end{figure} 
%%%%
%\textcolor{blue}{Include high quality pictures of needed data kinematics reach and expected proton images for unpolarized and polarized protons. Develop similar imaging for light nucleus, $d$ and $^4He$. }

\subsection{Overview}
\label{sec:GPDoverview}
Generalized Parton Distributions (GPDs) are hybrid objects that,  on one side, are similar to the parton distribution functions (PDFs) from  deep inelastic scattering (DIS) describing quark and gluon distributions in the longitudinal momentum fraction, $x$, at a given scale, $Q^2$. On the other hand, alike the nucleon elastic form factors (FFs), they give insight on the  internal spatial distribution of its constituents. GPDs depend on two additional kinematic variables: $\xi$, known as the skewness parameter, and $t$, which are respectively proportional to the longitudinal and transverse components of the momentum transfer variable, $\Delta$. Quark and gluon spatial probability distributions in the impact parameter, $b$, $q(x,b)$, are then obtained by Fourier transformation with respect to the transverse component $\Delta_T$, where, $\Delta_T^2 = -t$ at $\xi=0$. 
%
%
Most importantly, the distributions $q(x,b)$,  can be interpreted as specific projections of relativistic Wigner phase-space distributions. The latter give the most complete information on the proton's internal dynamics (for review papers we refer the reader to Refs.\cite{Diehl:2003ny,Belitsky:2005qn,Kumericki:2016ehc}). 
%

Being able to simultaneously describe both the spatial and momentum distributions of partons is a necessary step towards understanding the intriguing questions of how quarks and gluons are spatially organized to form the proton and neutron, and what gives origin to nucleon spin, as well as its other mechanical properties such as pressure and shear stress, based on quark-gluon interactions.
%
GPDs provide the theoretical backdrop in this context since they  parametrize the quark and gluon off-forward correlation functions in QCD. The Mellin moments of specific GPDs can then be used to define angular momentum as well as the other mechanical properties defining the internal structure of the proton \cite{Ji:1996ek}. 
%
In Refs.\cite{Ji:1996ek,Ji:1996nm} Ji defined a connection
that has revolutionized modern hadronic physics by introducing  the observable that brought for the first time partonic orbital angular momentum within experimental grasp, specifically with the cross section for the process of deeply virtual Compton scattering (DVCS).  The matrix elements for the DVCS process can, in fact, be described in terms of GPDs. 
A key step ultimately validating this new avenue was to ensure that QCD factorization was applicable as written in detail in Refs.\cite{Ji:1997nk,Ji:1998xh,Collins:1996fb}. 

The basic diagram and kinematics connecting the DVCS process to GPDs are illustrated in Fig.\ref{fig:dvcs} where the virtual exchanged by the lepton probe is on the left and a real photon is produced on the right. Deeply virtual Compton scattering (DVCS) is the prototype for all deeply virtual exclusive scattering (DVES) experiments, including deeply virtual meson electro-production (DVMP) where a meson replaces the outgoing photon in Fig.\ref{dvcs}, as well as crossed channel experiments such as timelike Compton scattering (TCS) where the initial photon is real, and the outgoing one is virtual, producing a lepton pair. Recently the possibility of pursuing double DVCS
(DDVCS) where both the initial and final photons are virtual, as well as %share similar QCD factorization properties as the DVCS process. 
other multi-particle production processes has also emerged. The latter ensure a more complete kinematic coverage of the variables needed to fully define GPDs.
%
%% add MASS
%Moreover, GPDs enabled us to access new quantities, such as the Gravitational Form Factors (GFFs) parameterizing the partonic energy momentum tensor (EMT), fundamental to the distributions of mass, angular momentum, and partonic forces. These new perspectives shed a refreshing new light on the problem of proton structure and confinement.

%%%%% 
%%%%%
\begin{figure}[htb!]
\centering
\includegraphics[width=0.4\columnwidth]{figures/dvcs.png}
\caption{The DVCS process in leading twist approximation. A virtual photon couples to a quark in the proton and the quark emits a high energy real photons in the final state. }
\label{fig:dvcs}
\end{figure}
%%%%%
%%%%%
%Other related channels such as deeply virtual meson production (DVMP), timelike Compton scattering (TCS) where a lepton pair is produced in the final state, as well as double DVCS  (DDVCS) where both the initial and final photons are virtual, share similar QCD factorization properties as the DVCS process. 
%Recently the possibility of pursuing multi-particle production processes has also emerged.
%
Finally, {\color{blue} electron-nucleus scattering} will give access to various spin configurations, including spin 0 ($^4He$) and spin 1 (deuteron), as well as unique information on the role of the initial stages of heavy ion collisions.     

To extract GPDs with sufficient accuracy from DVES experiments where three or more particles are detected in coincidence in the final state, requires very high luminosity to attain statistical precision, as well as a comparable systematic precision. The latter {\color{blue} requires carefully optimized specific instrumentation}. 
%The prototype diagram for a typical DVES process, deeply virtual Compton scattering (DVCS), is shown in Figure~\ref{dvcs}.   

Information on GPDs will be extracted from the simultaneous analysis of the various DVES processes, albeit each one with their own characteristic kinematic settings and behavior. 
The EIC experimental program on exclusives will extend the measurements obtained at Jefferson Lab, centered on DVCS and DVMP in the large $x_{Bj}$ region ($x_{Bj} \geq 0.2$) and $Q^2$ in the multi-GeV range, to the region of very low values of $x_{Bj}$  {\color{blue}  ($10^{-5} \leq x_{Bj} \leq 10^{-2}$)}.
%where sea quarks and gluons become the dominant component. 
One of the goals of the EIC at lower energies will be to probe the {\it transition} from the kinematic region dominated by valence quarks, to the sea quarks and gluons dominated one, by providing access to an intermediate range of $x_{Bj}$ values {\color{blue}($10^{-3}\leq x_{Bj} \leq 10^{-1}$)}. This transition will be monitored by tracking the $Q^2$ dependence of GPDs as the sea quarks and heavy flavors enter the picture. The corresponding description in coordinate space will provide unprecedented new information. 

DDVCS as well as multi-particle exclusive processes, in principle, {\color{blue} will allow access the kinematic domain}  
at $x \neq \pm \xi$. The price to be paid for extending the kinematics reach is a much reduced production rate compared to DVCS, due to the increased number of particles to be detected in coincidenc. 
%To my knowledge there are no simulations of that process available for the EIC energies and kinematics although 
%
Preliminary simulations for both JLab@12 and CLAS12 kinematics indicated that a viable contribution of DDVCS to the imaging program would require a 100-fold increase in luminosity compared to the DVCS rate. 
The experiments suggested for JLab@12 in the valence quark domain before the EIC becomes operational may be used to constrain the processes in the  $x \neq \pm \xi$ kinematics at the EIC.  

In what follows, after a description of the main physics goals, we outline a roadmap listing, step-by-step, the requirements for extracting GPDs from experimental data, using input from phenomenology and ab initio calculations, with sufficient accuracy to provide 3D images of the proton.  

%

\subsection{Roadmap for Reconstructing 3D quark and gluon images at EIC}
\label{sec:2B}
%In this section we address, on one side, the formalism for the cross section and the various spin asymmetries which contain the Compton Form Factors (CFFs) as observables used to ultimately extract GPDs from data. 
In order to reconstruct spatial images of the proton and to extract the matrix elements of the EMT from data, a multi-prong  effort is needed that combines observables from DVES, existing data from inclusive DIS and from elastic scattering, as well as information on both moments and $x$ dependent spectra of GPDs from lattice QCD.    

Furthemore, new state of the art computational methods and techniques are necessary to address the many layers of analysis used to extract the signal in its complex background after the large and diverse experimental data sets are acquired.
ML methods are currently being explored and will be implemented in order to handle the complex problem of coordinating the information from all the various inputs contributing to resolving 3D parton distributions. An interesting aspect of nuclear femtography is that the problems that need to be solved with computational methods, for instance, the inverse problem to extract GPDs from data, represent interesting challenges for ML experts. This has been generating an unprecedented wealth of continuously growing, truly collaborative efforts between nuclear physicists and computer scientists. 

The essential research sectors that define nuclear femtography, and that are being continuously developed, include:
\begin{itemize}
\item Theory of GPDs and Wigner distributions 
\item Observables and Data Extraction
\item Machine Learning approaches
\end{itemize}


\subsubsection{Theory of GPDs and Wigner Distributions}
\label{sec:IIIB1}
%\begin{itemize} 
%\item some intro and general concepts
%\item cross section for various processes and sensitivity to various GPDs including twist three
%\item so far only valence region, reaching for a full flavor decomposition 
%\item pqcd and twist expansion: address issues in a positive way in the sense that experiment will help elucidating
%\item Two prong effort: 1) Wigner distributions and how to access them. What are the issues, and efforts in similar kinematic settings (elastic scattering)
%\item 2) Can one extract $J_u$ and $J_d$ (integrated quantities/moments)
%\item Low $x_{Bj}$ vs. large $x_{Bj}$ 
%\end{itemize}

%We need a figure like \ref{fig:IR2kin_example}
%\vspace{0.3cm}

% Various GPDs describe different relative polarization configurations of the struck quark/gluon and proton.

\noindent GPDs enter the cross section for DVES at the amplitude level, encoded in the Compton Form Factors (CFFs) which, at a given scale, $Q^2$, are functions of the momentum transfer between the initial and final proton, parametrized by the variables $\xi$ and $t=\Delta^2$, where $\Delta =p'-p$ is the momentum transfer between the initial and final proton. QCD factorization theorems supporting this description are applicable in the $-t/Q^2 << 1$ limit. {\color{blue} In experimental analysis the constraint $-t/Q^2 < 0.2$ is often used.} 
In what follows we focus on the DVCS process shown in Fig.\ref{fig:dvcs}. DVCS can be considered the prototype for all DVES experiments and as such it's been the most studied process.
%%
The matrix elements DVCS are accessed through exclusive photoproduction, 
\[ e + p \rightarrow e' + p' + \gamma \]
where the final photon is produced at the proton vertex. A competing background process given by the Bethe-Heitler (BH) reaction is also present, where the photon is emitted from the electron and the matrix elements measure the proton elastic form factors. The cross section is a function of four independent kinematic variables besides the electron-proton CoM energy, $\sqrt{s}$: the scale, $Q^2$, the skewness, $\xi$,  related to Bjorken $x$ as $\xi \approx x_{Bj}/(2- x_{Bj})$, $t$, and the angle between the lepton and hadron planes, $\phi$. The two processes along with the relevant kinematic variables are shown in Figure \ref{fig:kinematics}.
%%%%%%%%%%%%%%%%%%%%% FIGURE KINEMATICS
\begin{figure}[htb!]
\begin{center}
\includegraphics[width=6cm]{figures/DVCS1.png}
\includegraphics[width=6cm]{figures/DVCS_Final.png}
\caption{Kinematics setting for the DVCS (right panel) and BH (left panel) processes.}
\label{fig:kinematics}
\end{center}
\end{figure}
%%%%%%%%%%%%%%%%%%%%
The CFFs are complex quantities which at leading order in perturbative QCD, are defined through the convolution integral,
\begin{eqnarray} 
\label{eq:GPD-CFF}
{\mathcal F}(\xi,t; Q^2)   =   
\int_{-1}^{1} dx \left[ \frac{1}{\xi-x-i\epsilon} -  \frac{1}{\xi+x-i\epsilon} \right] F(x,\xi,t; Q^2)  ,%\nonumber  
\end{eqnarray}
%where the real function of 3 parameters $H(x, \xi, t)$ is replaced with the complex function of 2 parameters 
%${\mathcal{H(\xi, \it t) }}$, and  
%$\text{Re} {\mathcal H(\xi, \it t)}$ and $\text{Im}{\mathcal H}(\xi,\it t)$, which can be determined experimentally.
where $\mathcal{F} = \mathcal{H}, \mathcal{E}, \widetilde{\mathcal{H}}, \widetilde{\mathcal{E}}$. 
Beyond the leading order the structure of the CFFs kernels in the square bracket in Eq.(\ref{eq:GPD-CFF}) representing Wilson coefficient functions for the off-forward process, becomes $Q^2$ dependent \cite{}.

Figure~\ref{fig:CFF} displays estimates of $ x_{Bj} \text{Re}{\mathcal H}$ and $x_{Bj} \text{Im}{\mathcal H}$ at fixed value of $t$. More about the evaluation.

%%% polarization observables?
%An example of what may be achieved 
%at the EIC with all polarization observables measured with high precision ({\color{red} to be defined}) (and in a large $\xi$ and $t$ range is shown in Fig.~\ref{quark-H-E}.
%%%%%%
%%%%%% FIGURE CFFs
%%%%%%
\begin{figure}[htbp]
\centering
\includegraphics[width=0.49\columnwidth]{figures/Im-H.png}
\includegraphics[width=0.49\columnwidth]{figures/Re-H.png}
\caption{Left: The imaginary part of the Compton Form Factor $\cal{H}$ extracted from simulated DVCS events with the tracking resolution given by the all-Silicon tracker. The bands for the EIC indicate the uncertainties due to overall reconstruction effects, statistics and systematic uncertainties. Right: The real part of the Compton Form Factor $\cal{H}$ extracted from simulated DVCS events. The bands for the EIC indicate the uncertainties due to overall reconstruction effects, statistics and systematic uncertainties. {\color{blue}A combined  integrated luminosity of $200fb^{-1}$ shared between longitudinally polarized and transverse polarized proton runs has been assumed}}
\label{fig:CFF}
\end{figure}

In order to reconstruct 3D images of the proton one faces two major challenges: 1) one needs to process multi-dimensional data; 2) the inverse problem. In order to attack both problems, it is important to have a detailed and accurate knowledge of the $t$-dependence of the CFFs in the measurable region, as well as to develop extrapolations methods to large values of $t$ needed for Fourier transformation. 

The first step towards these goals is to determine 2D projections in impact parameter space for different quark $x$ and $Q^2$. The quark and gluon densities are defined as \citep{Soper:1976jc,Burkardt:2000za,Ralston:2001xs,Diehl:2002he,Belitsky:2003nz,Liuti:2004hd,Lorce:2011kd},
\begin{eqnarray}
\rho^{q}_{\Lambda\lambda}({\bf b}) = H_{q}({\bf b}^2) + \frac{b^i}{M} \epsilon_{ij} S_T^j \frac{\partial}{\partial b} E_{q}({\bf b}^2) +  \Lambda \lambda \widetilde{H}_{q}({\bf b}^2),
\end{eqnarray}
where $i=1,2$, and $S_T^i$ is the transverse proton spin.  
$H_{q}({\bf b}^2), E_{q}({\bf b}^2)$, $\widetilde{H}_{q}({\bf b}^2)$,  are the Fourier transforms in the transverse plane of the $t$-dependent GPDs corresponding to different quark-proton polarization configurations.  

The four-momentum transfer squared $t$, is related to the transverse momentum transfer, ${\bf \Delta}_T$ as: $t = t_0 - {{\bf \Delta}_T^2}/({1-\xi^2})$, where $t_0 = - {4 \xi^2 M^2}/({1-\xi^2})$, and $\xi$ is the fraction of longitudinal momentum transfer. 

Tomographic images of the structure of the proton in 3D are obtained, in principle, from momentum slices of successive spatial parton distributions. 

A new generation of current and planned experiments at the future EIC could in principle allow us to incorporate all the information from data and phenomenology into a tomographic image connecting the deepest part of the quantum world with what we see as everyday matter around us. 
%However, each experiment can only add a small piece to the picture. To increase the reach of this emergent field there is an urgent need to harness and organize information from experiment. 
This will require going beyond standard computational methods and addressing the computational challenges that are presently limiting our access to the proton’s 3D structure.

{\bf Here I want to quote also importance of lattice, Mantysaari and Dupre picture}.
Modeling and using lattice QCD to simultaneously develop a flexible model of the Wigner distribution which underlies the theoretical description of the data will also be necessary.

Flexible parametrization including valence, sea quarks and gluon components which can be perturbatively evolved to the scale of the data are needed for the analysis. 

They should be able to build on the previously determined valence distributions at Jlab which are modeled at a low initial scale in the $GeV$ region. At this scale only valence quarks are present. 
{\bf and extend to gluons and sea quarks (quark-antiquark pairs) resolved as independent degrees of freedom at a larger scale.} 

The phenomenology of perturbative QCD evolution is therefore similar to the one extensively developed for inclusive scattering. The observables, the Compton Form Factors (CFFs), are complex quantities obtained as convolutions of GPDs with kernels governed by perturbative QCD. 

Notwithstanding this additional complication, the quark, antiquark and gluon components of CFFs and consequently of GPDs, can be extracted from deeply virtual exclusive experiments with the same logic behind DIS, {\it i.e.}  merging information from a combination of electron and neutrino probes, including meson production, {\it e.g.} $J/\psi$ production which is sensitive to the gluon content (see reviews in \cite{Kumericki:2016ehc,Lin:2020rut}), and crossed channel experiments such as deeply virtual exclusive pion-proton Drell Yan scattering \cite{Sawada:2016mao,Chang:2020rdy}.
% 
While present available data sets cover somewhat limited kinematic ranges which are neither sufficient to separate out the various components, nor to gauge their relative importance in the various regions, the exclusive program at Jefferson Lab@12 GeV, as well as upcoming measurements at COMPASS and JPARC will provide, in the upcoming years, a large amount of precise data. A wide range of diverse experiments from various targets will be performed, from DVCS, to timelike Compton scattering (TCS), and various meson production processes. The future planned Electron Ion Colliders (EIC, EIcC), will further these exploration at both higher four momentum transfer squared $Q^2$ and low Bjorken $x_{Bj}$. 

-- use of lattice

%CFF only provides the 2D information. To recover the 3D, one either needs $Q^2$ evolution, or additional data from lattice QCD computation.

The cross section terms for each beam-target polarization configuration ...Several CFF combinations corresponding to various quark-proton polarization configurations appear simultaneously in  \cite{Kriesten:2019jep}. 
Measuring the DVCS process with polarized electrons (and positrons), and with longitudinal and transverse polarized protons at high integrated luminosity will allow for the extraction of the Compton Form Factors (CFF) $\cal{H}{\xi, \rm t)}$, $\cal{E(\xi,\rm t)}$, and $\tilde{\cal{H}}(\xi, \rm t)$.

%, where $\xi \approx x_B/(2-x_B)$. (already defined)

%
%
%%%% TCS
%GPDs are difficult to directly extract from DVCS measurements, and a direct extraction is limited to the kinematics of $x = \pm \xi$. A more complete kinematics coverage is possible if the final state real photon in Fig.~\ref{dvcs} is replaced by a time-like virtual photon as $$e^- p \to e^- p  \gamma^* ~~(\gamma^* \to e^+ e^-)$$. 

%%%% DDVCS
%The double-DVCS process is several orders of magnitude reduced in rate compared to DVCS making it accessible at high enough rates only at much higher instantaneous luminosity than will be available at the EIC.  
%




{\it Twist-3 GPD, Light Nuclei, ETC...}

why do we need twist-3? is it possible for EIC to extract twist-3 GPDs? 


%Access to the Generalized Parton Distributions is key to constructing 3D images (2D in coordinate space, 1D in momentum space). 
  
%\begin{figure}[h]
%\centering
%\includegraphics[width=0.80\columnwidth]{figures/Quark-bx-by.png}
%\caption{Left column: Transverse impact parameter distribution of quarks in 
%a transversely polarized proton. Quark distribution of a proton polarized 
%transversely and projection onto the $b_x$ axis. The distribution is dominated by GPD H. 
%Right column: Same at left but for the GPD E only. E projects out the angular momentum distribution inside the proton. It shows the shift in $b_y$ of the quark charges due to
%the orbital angular momentum contribution. }
%\label{quark-H-E}
%\end{figure}
      
%{\color{blue} This relationship is expressed through the -t dependence of $d_1(t)$~\cite{Polyakov:2018zvc}, 
%which may be determined from the DVCS data~\cite{Burkert:2018bqq}. Estimates for Re{$\mathcal{H}$} and Im{$\mathcal{H}$} 
%from measuring DVCS in different polarization states and with both electron and positron beams, are shown 
%in Figure~\ref{CFF}. Knowledge of the CFF $\cal{H}$ in a large range of $\xi$ $Q^2$ and $-t$ enables extraction of 
%the gravitational FF $d_1(t)$, a prerequisite for determining the mechanical properties such as shear forces and 
%internal pressure distributions. The Compton Form Factor Re$\cal{H}$ can be related to the mechanical properties of the proton such as shear forces, pressure distribution and its mechanical radius~\cite{Polyakov:2002yz}. \\

%Data obtained from employing transverse polarized protons in addition to longitudinal polarized protons, and including
%positron beam, also enables the 
%determination of the CFF $\cal{E}$ in a large kinematics range. Together with $\cal{H}$, $\cal{E}$ is sensitive to 
%the gravitational FF $J(t)$ and the orbital angular momentum spatial distribution in the proton. To determine this 
%fundamental quantity is a primary goal of the EIC program. It will require both precision studies of DVCS at high CM energies and at low CM energies to completely cover the full EIC kinematics space with precision data and to connect
%it to high precision fixed target experiments covering the full valence region. }

\subsubsection{Observables and GPD extraction}
\label{sec2p1}
Deeply virtual exclusive processes have been identified as the cleanest experimental probe of the 3D structure of the proton as well as its mechanical properties including the quark and gluon distributions of angular momentum, pressure, and shear forces (see reviews in \cite{Goeke:2001tz,Diehl:2001pm,Belitsky:2005qn,Kumericki:2016ehc}). 
%%%%%
%%%%%
%%%%% 
%%%%%
\begin{figure}[htb!]
\centering{
\includegraphics[width=1.0\columnwidth]{figures/EIC-5x41-xB-t.png}}     %JRA - updated file name to avoid compilation errors - plot is consistent with caption, but there may be plan to modify...
%\includegraphics[width=1.0\columnwidth]{figures/EIC-kinematics-5x41.png}}
\caption{VB: {\color{blue} Accessible kinematics and event rates for the DVCS process at center-of-mass energies $\sqrt{s}=28$~GeV for $Q^2$ vs $x_B$ (left), and for the azimuthal angle $\phi$ versus 4-momentum transfer -t (right).The color code indicates the number of events per $Q^2$-$x_B$ pixel and for $\phi$-$t$ pixels, respectively. {\bf Need to include integrated luminosity. Do we need other kinematics graphs, e.g. angular distributions?} } }
\label{fig:IR2kin_example}
\end{figure}
%%%%%
%%%%%

%The standard approach of imaging is through diffractive scattering, as in optics. 
To obtain phase-space quark and gluon information, a new type of diffractive scattering was proposed in which a deeply-virtual photon, with virtuality much larger than any other scale, diffracts on a nucleon, generating a real photon or other hadrons~\cite{Ji:1996ek}. 
%(see Fig. \ref{fig:dep}). 
The real photon production process has been called deeply-virtual Compton scattering or DVCS~\cite{Ji:1996nm}, and for meson production, deeply-virtual meson production (DVMP)~\cite{Radyushkin:1996ru}.
DEPs contain the elements to learn the origin 
of the nucleon mass and spin, and its mechanical properties, such as pressure, and shear forces. The information on these fundamental physical properties appears encoded in the %Generalized
%Parton Distributions 
GPDs.

Deeply Virtual Compton Scattering (DVCS) is a key exclusive process that enables to access information about the Generalized Parton Distributions~\cite{Ji:1996nm}. 
This reaction has been measured at various laboratories employing lepton beams. The current program at Jefferson Lab is the most advance program employing intense electron beam, of up to 12~GeV energy at $10^{35}$cm$^{-2}$sec$^{-1}$ luminosity with the large acceptance detectors CLAS12 and over $10^{37}$cm$^{-2}$sec$^{-1}$ luminosity in focusing magnetic spectrometer based setups with more limited acceptances. These experiments cover the range $x_B > 0.1$. 

The EIC with its much larger energy reach, and employing polarized electrons and polarized protons, both longitudinally and transversely polarized, at instantaneous luminosity of up to  $10^{34}$cm$^{-2}$sec$^{-1}$, we enter into the high-precision phase of DVCS, and cover a much larger range in $x_B>10^{-3}$. 

%The kinematic dependence of DVCS at the EIC kinematics is shown in Figure~\ref{EIC-kine1} for the EIC center-of-mass energy %at $\sqrt{s}=28$~GeV.    

%\begin{figure}[h!] 
%\includegraphics[width=0.4\columnwidth]{figures/EIC-kine-22GeV}
%\caption{{\bf this graph is a placeholder for a graph showing the EIC reach at different center-of-mass energies, to be made)} }   
%\label{EIC-kine1}
%\end{figure}

First, 
the Jefferson Lab (JLab) 12 GeV facility has come online. Of the approved proposals, roughly {\it one third 
of the experiments 
are generating large data sets from deep-exclusive processes} which are directly relevant to quark and gluon imaging. More data for gluons and sea quarks will come from the planned Electron-Ion Collider (EIC) at Brookhaven National Lab (BNL). Second, novel {\it ab initio} calculations from lattice QCD for large momentum nucleon states have produced a first glimpse of the isovector quark distributions in transverse space, and much more systematic and large scale calculations will be available in the exa-scale computation era (see, Sec.~\ref{sec:lattice}). Third, the application of Artificial Intelligence (AI) to nuclear femtography has now begun. The Center for Nuclear Femtography (CNF) at Southeastern Universities Research Association (SURA) in DC has recently been created to respond to the challenge of generating tomographic images of the nucleon. In the last two years, CNF has been actively exploring methods and opportunities by funding several experimental and theoretical groups working on AI-assisted 
image generation. The framework has been set up
and the groundwork has been laid for turning the dream of nuclear femtography into a reality.


%Mapping the 3D images of the nucleon in terms of GPDs
%These femto-scale images (or femtography)
However, obtaining high-quality images from experimental data has remained a dream for more than two decades.  
First, one would need to have a large amount of a specific type of experimental data---deep exclusive processes (DEP)---from high-energy electron-nucleon collisions, which has not been available. Second, as in any other imaging process, turning the data into images requires algorithms that can efficiently extract critical information from them. In the case of nucleon femtography, this represents a big challenge that has not yet been met, and that this proposal aims to overcome. 
 
Each aspect of the physics program can in principle be applied
to define its own idealised detector design and configuration


\noindent Experimental Probes at EIC

What experimental measurements are needed with what final states ($p\gamma$, $pJ/\psi,p\phi?$) including different polarization of initial states? Flavor separation, nuclear target, singlet \& non-singlet contributions

%DVCS. 

%meson production, heavy flavors


%What does a positron beam add in sensitivity?

 Beam and target single-spin dependent cross sections are proportional to the imaginary part of the interference amplitude. Thus the difference of polarized electrons or polarized positrons DVCS cross sections gives nearly direct access to the imaginary part of the CFFs, which are in turn equal (at leading order) to the GPDs on the {\it diagonal} $x$=$\pm \xi$. In addition, the DDVCS process which involves a final time-like virtual photon allows to access the $x \neq \pm \xi$ phase-space~\cite{PhysRevLett.90.012001,PhysRevLett.90.022001}.  Beam-charge dependent observables in the DVCS reaction have the unique property to isolate the contributions from the real-part of the interference amplitude~\cite{CLAS:2021gwi}. {\color{blue} Implementing positron beams in the EIC would significantly enhance its capabilities in the high impact 3D imaging science program. }  

While beam and target single-spin asymmetries are proportional to the imaginary part of the $DVCS$-$BH$ interference amplitude, accessing the real part is significantly more challenging. It appears in the unpolarized cross sections for which either the $BH$ contribution is dominant, or all three terms (pure $BH$, pure $DVCS$, and interference amplitudes) are comparable. The $DVCS$ and interference terms can be separated in the unpolarized cross-sections by exploiting their dependencies on the incident beam energy, a generalized Rosenbluth separation. This is an experimentally elaborated procedure, and necessitates some theoretical hypothesis to ultimately extract an ambiguous physics  content~\cite{Defurne:2017paw,Kriesten:2020apm}. The real part also appears in double-spin asymmetries, but these can receive  significant direct contribution from the BH process itself, and are also experimentally challenging. Unpolarized BCAs are directly proportional to the real part of the $INT$ term, and receive no direct contribution from the BH process. As such they provide the cleanest access to this crucial observable, without the need for additional theoretical assumptions in the CFFs extraction procedure.


{ \it What are the cm energy and integrated luminosity requirements for precision imaging}

\textcolor{red}{How do we know this, how do we get information on this? We are limited by the systematics of the extraction method, in the various methods/approximations used. We can insert evaluations based on ML approaches.}
\textcolor{blue}{VB: I think it would be a mistake to limit the data volume just because at the present time the systematics may be dominated by the currently available extraction method. But this may change with improvements in our ability to develop theoretical constraints, or exploit LQCD to "measure" certain quantities the lack of knowledge of those may currently dominate the systematic uncertainty. Analysis techniques will always improve, the data volume remains the same.} 

%%%%% 
%%%%%
\begin{figure}[htb!]
\centering
\includegraphics[width=0.6\columnwidth]{figures/24GEV_Energydep.png}
\caption{Energy dependence of the ratio of the DVCS-BH interference term over the BH background. This graph was done for the Jlab@24 GeV kinematics and it should be replaced by an analogous one for the EIC second IR kinematics.}
\label{dvcs}
\end{figure}
%%%%%
%%%%%

\textcolor{red}{Importance of error analysis: we need to address the question of what precision of the experimental data is needed to be able to extract Wigner distributions with their full spatial coordinate dependence.
}
\begin{itemize}
\item The error in the cross section generates a larger error on the various CFFs depending on what process we use to analyze them. What are the quantitative studies that have been done so far addressing this issue? What graphs can we insert?
\item The EIC will run after Jlab@12 GeV, there are two scenarios, with Jlab@24 GeV and without. Barring the Jlab@24 GeV possibility we have (???) {\color{blue}VB:  I don't think we should refer to 24 GeV, it is not a real project (yet)}
\end{itemize}



{\color{green}LE\subsubsection{AI/ML fitting} Let us move this part to the AI section and combine it with the existing pargraph
\label{sec:IIIC}
Artificial Intelligence (AI) methods including  machine learning (ML), have been increasingly applied to attack several of the outstanding questions in QCD,  ranging from the sign problem \cite{Ohnishi:2019ljc,Mori:2017pne,Alexandru:2018fqp}  to the inverse problem in lattice QCD. Furthermore, ML methods have been recently applied to extract the behavior of parton distributions functions (PDFs) from data (NNPDF). 
%
%
Nevertheless, the systematic application of AI to problems in hadronic physics can still be considered to be in its initial stages. 
One important aspect that is still being developed concerns the treatment of uncertainty, in particular, studying the accuracy of AI based predictions within a well defined statistical approach and with precise benchmarking.

This is particularly important for the science of nuclear femtography that aims at reconstructing the spatial structure of hadrons, or nucleon tomography, using information from deeply virtual electron proton exclusive photoproduction, $ e p \rightarrow e' p' \gamma$, and various other related reactions. Open questions are the choice of a ML method that is suitable to attack the issues specific to nuclear femtography, including the impact of noise and experimental uncertainty.

The complexity associated with the large number of kinematic variables, and the complex structure of the cross section makes the problem of extracting tomographic images of quark and gluon structure of the proton virtually impossible to solve with traditional methods; for high precision femtography, which is required to obtain proton images, we need to develop more sophisticated analyses. The success of ML methodologies in modeling complex natural phenomenon make this a prime choice for GPD extraction.}

==> IR.tex <==

\section{EIC Interaction Regions and Luminosity}% (R.\ Gamage, Y.\ Zhang, V.\ Morozov, \underline{T.\ Satogata)}}
{.}

%\begin{itemize} 
%\item 
%What modifications and R\&D is required from the baseline design version to achieve the highest luminosity in the range of  $\sqrt{s} = 20 - 45$~GeV strong focusing?, strong hadron cooling?, ....etc    
%\end{itemize}

The capability of having two interaction regions (IRs) is one of the EIC design requirements. This section discusses implementation of a second IR consistent with nuclear physics, accelerator, and engineering requirements. These include the operation of both IRs over the entire energy range of $\sim 20\,{\rm GeV}$ to $140\,{\rm GeV}$ center of mass. The second IR can also provide a different acceptance coverage than the first IR. This section also includes consideration of different modes of IR operations and their effects on beam dynamics.

The luminosity and the design of the reference first EIC interaction region is optimized emphasizing the discovery potential of the EIC by providing the highest luminosity near the upper end of the CM energy range, from $\sim 80\,{\rm GeV}$ to 120\,GeV, while covering the entire range of parameters required by the Nuclear Physics Long Range Plan.  The parameter set and design is based on 1160 colliding bunches in each beam:
\begin{itemize}
\item{Peak luminosity of $L=10^{34}\,{\rm cm}^{-2}{\rm s}^{-1}$ at a center-of-mass (CM) energy of 105\,GeV;}
\item{Crossing angle $\theta_c=25\,{\rm mrad};$}
\item{Maximum $\beta$-functions in the low-$\beta$ quadrupole magnets, $\beta_{\rm max} \leq 1800\,{\rm m}$ (for protons in the vertical direction)  
  and acceptable nonlinear chromaticity resulting in
  sufficient dynamic aperture;}
\item{IBS growth times in horizontal and longitudinal directions of $\tau_{\rm IBS} > 2\,{\rm hours}.$}
\end{itemize}

The overall EIC layout is sufficiently flexible to allow for alternative optimization. The IRs may be optimized at different CM energies. Moreover, the two IRs and corresponding detectors may be optimized for different parts of the physics program. Here the second IR is optimized for operations and luminosity production in the EIC central CM energy range.

To first order, the luminosity at the IP is inversely proportional to the distance between the last upstream and first downstream final focus quadrupoles (FFQs). The statistical uncertainty of measurements in the central detector scales as this distance. However, the closer the beam elements are to the IP, the more they obstruct the acceptance at shallow angles with respect to the beam axis and restrict the acceptance for forward particles. The solenoidal field used in the central detector region to measure the high $p_T$ particles in the central detector is not effective in determining the momenta of particles moving parallel to the beam direction, and additional fields are needed. 

From kinematics, the reaction products are biased towards small angles around the original ion beam. In particular, the detection of small-angle products requires acceptance to the recoiling target baryon (3D structure of the nucleon), hadrons produced from its breakup (target fragmentation), or all the possible remnants produced when using nuclear targets (including the tagging of spectator protons in polarized deuterium). The detection has to be done over a wide range of momenta (and charge-to-mass ratios) with respect to the original ion beam. The second IR design must overcome these measurement difficulties posed by the beam elements.

From machine design and luminosity considerations, it is not desirable to leave a very large detector space free of beam focusing elements to allow the small-angle products to accumulate sufficient transverse separation from the incident beams. The solution is to let the small-angle particles pass through the nearest elements of the machine final-focusing system, which simultaneously perform the function of angle and momentum analyzer for the small angle reaction products. A significant challenge of this approach is to balance often contradictory detector and machine optics requirements.  

The above detection requirements make the detector and machine designs intertwined and closely integrated. There is no longer a clear separation between the detector and machine components. Several detection parameters directly impact the design choices for the second IR and vice versa. The major parameters critical to both detector and machine aspects of the design are summarized in Table~\ref{tab:2ndIRreqs}. Table~\ref{tab:2ndIRreqs} also provides a comparison of the second IR parameters to those of the first IR.

\begin{table}[htb]
%\begin{sidewaystable}[ht]
\begin{center}
\vspace*{1mm}
\caption{Summary of second IR design requirements and their comparison to the first IR. \label{tab:2ndIRreqs}}
%\renewcommand{\arraystretch}{1.4}
\small{
\begin{tabular}{c|l|c|c|l}
\toprule
\# & Parameter & EIC IR \#1 & EIC IR \#2 & Impact \\
\midrule
1 & Energy range & & & Facility operation \\
  & ~~~electrons [GeV] & 5--18 & 5--18 & \\
  & ~~~protons [GeV] & 41, 100--275 & 41, 100--275 & \\ \hline
2 & CM energy range of & & & Physics priorities \\
  & optimum luminosity [GeV] & 80--120 & 45--80 & \\  \hline
3 & Crossing angle [mrad] & 25 & 25--50 	& $p_T$ resolution, \\
 & 					& 	& 		& acceptance, geometry \\ \hline
4 & Detector space  	& -4.5/+4.5 	& -(3.5--4.5)/ & Forward/rear  \\ 
   &symmetry [m] 	& 			& +(5.5--4.5) & acceptance balance \\ \hline
5 & Forward angular & 20 & 20--30 & Spectrometer dipole aperture	\\ 
 & acceptance [mrad] & 	&		 & 						\\ \hline
6 & Far-forward angular & 4.5 & 5--10 & Neutron cone, Max. $p_T$ \\ 
  &  acceptance [mrad] &        &           &   						\\ \hline
7 & Minimum $\Delta(B\rho)/(B\rho)$  & & & Beam focus with dispersion, \\
  & allowing for detection  & 0.1 & 0.003--0.01 & reach in $x_L$ and $p_T$ resolution, \\
  &  of $p_T=0$ fragments & & & reach in $x_B$ for exclusive proc. \\ \hline
8 & RMS angular beam diver-   & 0.1/0.2  	& $<$0.2 	& Min. $p_T$, $p_T$ resolution \\
  & gence at IP, h/v [mrad] 	& 			&	 	& 				\\ \hline
9 & Low $Q^2$ electron acceptance & $<$0.1 & $<$0.1 & Not a hard requirement \\ 
\bottomrule
\end{tabular}
}   % \small
\end{center}
%\end{sidewaystable}
\end{table}

\begin{enumerate}
    \item Clearly, the second IR must at least be able to transport both beams over their entire energy ranges for operation of the facility to its entire potential. This first of all means that all dipole magnets in the second IR must have sufficient field integrals to provide the necessary bending angles keeping the IR footprint fixed from the lowest to the highest energy. The quadrupoles must also be strong enough to provide sufficient focusing to properly transport the beam in the entire energy range. This in turn means that none of the second IR magnets can have aperture-edge fields higher than 4.6~T at the top energy. It is of course desirable to operate the second IR in the collision mode. The second IR dipoles and quadrupoles must then have sufficient strengths to focus the beams at the IP while having sufficient large apertures to meet the detection requirements discussed below. Simultaneous operation of the two IR is also subject to the beam dynamics constraints discussed below.

\item Consistent with user demands and the two detector complementarity approach, the second IR is optimized to provide the highest luminosity at a lower CM than the first IR, between $\approx 45\,{\rm GeV}$ and $\approx 80\,{\rm GeV}$. This allows one to level off the luminosity curve of the EIC as a whole at a higher level over a wider energy range. It can also provide a different acceptance coverage than the first IR.

\item The ion and electron beams cross at a relatively large angle of 25--50~mrad at the IP. High luminosity is preserved through the use of crab cavities. This angle moves the ion beam away from the electron beam elements and makes room for dipoles located just downstream of the central detector area. The dipoles serve two purposes. First, they shape the beam orbits providing their geometric match, making the IR footprint fit in the available detector hall and tunnel space, and creating room for detectors. Second, the dipole systems allow momentum analysis of the particles with small transverse momentum with respect to the beams. The particles with large transverse momenta are analyzed using the solenoidal field in the central detector.
\end{enumerate}
\begin{figure}[ht]
    \centering
    \vspace*{1mm}
    \includegraphics[width=0.7\textwidth]
    {figures/crabtilt.png}
    \caption{Apparent smear of the beam spot size at the IP due to the crab tilt.}
    \label{fig:crabtilt}
      \vspace*{1mm}
  \end{figure}
The crabbing tilt of a bunch at the IP effectively smears the beam spot size seen by the Roman Pot (RP) detectors as illustrated in Figure~\ref{fig:crabtilt}. The effective beam spot size is one of the sources of uncertainty in a $p_T$ measurement. Ignoring for the moment other sources such as the beam angular spread at the IP, the transverse position of a scattered particle at an RP $x_{RP}$ is related to $p_T$ as
\begin{equation}
x_{RP} = M_{11} x_{IP} + M_{12} p_T /p ,
 \end{equation}
where $x_{IP}$ is the scattered particle's transverse position at the IP and $p$ is the beam momentum. $M_{11}$ and $M_{12}$ are elements of the linear beam transfer matrix from the IP to the RP known from the magnetic optics design:
\begin{eqnarray}
M_{11} & = & \sqrt{\beta_{RP}/\beta_{IP}}\cos\Delta\Psi , \\ \nonumber
M_{12} & = & \sqrt{\beta_{RP}\beta_{IP}}\sin\Delta\Psi ,
 \end{eqnarray}
where $\beta_{RP}$ and $\beta_{IP}$ are the Twiss $\beta$-functions at the RP and IP, respectively, and $\Delta\Psi$ is the betatron phase advance from the IP to the RP. The measured $p_T$ can be expressed as
\begin{equation} 
p_T = p \frac{x_{RP}}{\sqrt{\beta_{RP}\beta_{IP}}\sin\Delta\Psi}-p\frac{1}{\beta_{IP}}\frac{\cos\Delta\Psi}{\sin\Delta\Psi}x_{IP}.
 \end{equation}
Since it is challenging to measure $x_{IP}$ precisely, the second term on the right-hand side of the above equation represents a measurement uncertainty 
\begin{equation} \label{eq:ptuncert}
\Delta p_T = \left| p\frac{1}{\beta_{IP}}\frac{\cos\Delta\Psi}{\sin\Delta\Psi}x_{IP} \right |.
 \end{equation}
$x_{IP}$ consists of a random betatron component $x_{\beta}$ and a longitudinal-position-correlated component $z\,\theta/2$:
\begin{equation}\label{eq:xip}
x_{IP}=x_{\beta}+z\,\theta/2, 
 \end{equation}
where $z$ is the particles longitudinal position from the center of the bunch and $\theta$ is the total beam crossing angle.


The second term in Equation~\ref{eq:xip} describes the beam spot size smear. It is typically much greater than the first term. Therefore, the uncertainty term in Equation~\ref{eq:ptuncert} can be greatly reduced by measuring the event's $z$ position. It has been suggested that, with a feasible RP timing of $\sim 35$~ps, the $z$ position can be resolved down to $\sim 1$~cm. 

Another factor in the uncertainty term of Equation~\ref{eq:ptuncert} is $\cos\Delta\Psi$. By placing the RP at a position with $\Delta\Psi$ close to $\pi/2$, $\Delta p_T$ in Equation~\ref{eq:ptuncert} can in principle be made arbitrarily small. There may be practical considerations limiting the available choice of $\Delta\Psi$ such as the requirement of placing the RP before the crab cavities, which have small apertures and kick the particles. In the presented design of the second IR, $\Delta\Psi$ is adjusted as close to $\pi/2$ at the RP as allowed by other constraints to minimize $\Delta p_T$.

  
Physics simulations set a requirement on the contribution of the crabbing tilt to $\Delta p_T$ of
\begin{equation}\label{eq:dptreq}
\Delta p_T < 20~{\rm MeV}. 
 \end{equation}
\begin{figure}[ht]
    \centering
      \vspace*{1mm}
    \includegraphics[width=0.35\textwidth]
    {figures/rapiditygap.png}
    \caption{Gap in the electron rapidity coverage due to the crossing angle and the ion beam pipe. The blue and red circles represent the ion and electron beam pipes at the EM calorimeter location. The black dashed circle outlines the solid angle without full azimuthal detector acceptance.}
    \label{fig:rapiditygap}
      \vspace*{1mm}
  \end{figure}
Another issue with the size of the crossing angle is that it contributes to the gap in the electron rapidity coverage in the rear direction as illustrated in Figure~\ref{fig:rapiditygap}. There is no full azimuthal coverage within an angle defined by the crossing angle and the size of the ion beam pipe. Assuming 5~cm for the radius of the ion beam pipe at a 2.5~m distance in the rear direction from the IP, the total polar angle of the gap in the rapidity coverage is about 20~mrad$+\theta_{cr}$. 


%\clearpage

==> instrumentation.tex <==
{In this part describe the instrumentation requirements for the science highlight described in the WP }

==> introduction.tex <==
\section{Introduction}

We have known for half a century that protons and neutrons, the fundamental building blocks of ordinary matter in the universe, are composed of quarks and gluons, together known as partons. We also know that global properties of nucleons and nuclei, such as their mass and spin, and their interactions are the consequences of the underlying physics of quarks and gluons. Yet, we still do not understand how these properties emerge from these fundamental interaction. This has resulted in the development of a new science of emergent phenomena in nuclear material and 3D nuclear structure: nuclear femtography. A part of the science program currently at the Jefferson Lab 12GeV CEBAF facility is aimed at this new science in the range where valence quarks dominate the internal dynamics; the US Electron Ion Collider in its low to medium center-of-mass energy implementation enables the exploration of anti-quarks and gluons. 
These capabilities will open the door to the exploration of the three-dimensional distributions in euclidean and in momentum space of the quarks and gluons in the nucleon over an unprecedented kinematic range and linking on to the energy range currently explored at lower energies.  The combined result will be an unparalleled exploration of the way in which the phenomena of nuclear physics, the mass, and the spin, and the mechanical properties emerge from the fundamental interactions of the partons, and how these properties are distributed in the confined space inside of nucleons and nuclei.  

The EIC in a range of 20 to 100 GeV center-of-mass energy, and featuring high luminosity operation, will be an ideal facility for the exploration of the most intricate secrets of the strong interaction, and the potential discovery of phenomena not observed before. The compelling science program has been described in previous documents~\cite{}.      

\begin{figure}[ht!]
\centering{\includegraphics[width=0.8\columnwidth]{figures/EIC.png}}
\caption{The EIC concept at Brookhaven National Laboratory.  The electron and the ion beams are clearly identified. There are several beam intersection points, one at the 6 o'clock (IP6) location and at the 8 o'clock (IP8) location are suitable for the installation and operation of large scale detector systems. Interaction point IP8 may be most suitable for high-luminosity optimization at low to intermediate center-of-mass energies as well as for the installation of a secondary focus for forward processes requiring high momentum resolution. 
The ion beam is circulating counter clockwise, and the new electron ring with electrons circling clockwise. Both beams will be highly polarized with proton polarizations over 70\% and electron polarization over 70\% as well(~\cite{Willecke-talks}). The EIC will benefit from two existing large detector halls in IP6 and in IR8, both fully equipped with infrastructure.}
\label{EIC-concept}
\end{figure} 
\begin{figure}[!ht]
\centering{\includegraphics[width=0.6\columnwidth]{figures/EIC_lumi_2021.png}}
\caption{{\bf Replace with a cleaned-up version.} Estimated luminosity versus center-of-mass energies for the operation of one (thick lines) or two (thin lines) interaction regions. The blue lines show the baseline performance. The green lines show the high luminosity operation for improved beam optics and cooling. } 
\label{EIC-lumi}
\end{figure}
With this document we highlight the science benefiting from an optimized operation at instantaneous luminosity up to $10^{34}$~cm$^{-2}$s$^{-1}$ in a center-of-mass energy range $\sqrt{s} = 25 - 60$~GeV. Such luminosity has been estimated to be achievable with improved beam optics and internal beam dynamics, and this White Paper aims at highlighting the important benefits in the science reach of the EIC. 
We also aim at providing the justification for the development of IP8 with characteristics that will provide support for an exciting science program at low to medium-high center-of-mass electron-ion collisions that address many of the high impact physics topics. In particular, 
the 3D-imaging of the nucleon, requiring a large amount of data in order to fill the multi-dimensional space with high statistics data, including two combinations of electron and proton polarization. We also emphasize the importance of, in the future,  including positron beam for processes that can be isolated through the measurement of electrical charge differences. The availability of high spin polarization for both the lepton beam as well as for the protons in both the longitudinal spin orientation and in the transverse direction. The latter is critical for the measurement of the angular momentum distribution in the proton through the generalized parton distributions.      
 
 
%\subsection{Overview - The Science of the $2^{nd}$ Interaction Region} 

%In this section we describe the key components of the exciting science program for the second Interaction region. 
%It covers the new avenue of the exploration of gravitational structure of nucleons and nuclei afforded by novel
%theoretical developments of the gravitational form factors that enables 

%A general overview of the program is presented in table~\ref{science-overview}. 
%\begin{table}[!ht]
%\caption{A list of data sets to be acquired in the first phase of operation. It will deliver a substantial part of high priority physics outlined in the EIC Whitepaper [2]. Average luminosity of $10^{34}$~cm$^{-2}$~s$^{-1}$, corresponds to integrated luminosity per year of 100 fb$^{-1}$. The "L" and "T" indicate longitudinal or transverse electron and hadron polarization. The CM energies are shown for electron-proton (ep) operations. {\bf The entries in the table should be updated with new results from YR + INT-program studies.}}
%\vspace{0.5cm}
%{\large

%\vfill\eject
%\newpage 
%\begin{figure}[t!]
%\includegraphics[width=1.0\columnwidth]{EIC-WP-lumi-needs.png}
%\caption{\bf These numbers seem no longer realistic, make new table.}
%\label{EIC}
%\end{figure} 





==> z8-farforward-backupwithnotes.tex <==
\section{Science of far forward particle detection}
\label{sec:forward}

\subsection{Far-forward detection overview}

In contrast to colliders that are mainly built to study particles produced at central rapidities, much of the EIC physics critically relies on excellent detection of the target and target fragments moving along, and often within, the outgoing ion beam. Consequently, EIC detectors are from the outset designed with an elaborate far-forward detection system that is closely integrated with the interaction region of the accelerator. The forward detection has several stages: the endcap of the central detector, trackers within a large-bore dipole magnet in front of the accelerator quadrupole (quad) magnets, two sets of Roman pots (one for charged particles at lower rigidities, so-called ``off-momentum detectors"; the other for tagging protons or light ions near the beam momentum) after a larger dipole behind the quads as seen in 
Fig.~\ref{fig:IP6_FF_layout} which shows the layout of IP6 during the time of the Yellow Report, which is largely unchanged. Additionally, a zero-degree calorimeter is employed for tagging neutrons and photons at very small ($<$5 mrad) polar angles. 

This arrangement allows for high-$p_{T}$ cutoffs to be determined by the magnet apertures, such as is the case for the neutron/photon cone going toward the zero-degree calorimeter (which must traverse the full hadron lattice), and for charged particles and photons being tagged in the first, large-bore dipole magnet after the IP, which contains a detector for far-forward particles at polar angles roughly between 5.5 and 20\,mrad. The bore of the first dipole (called B0pf in IP6) has a radius of 20\,cm (while the pre-conceptual design for IP8 has an equivalent dipole magnet with a slightly larger radius), which in principle allows for larger acceptance than 20 mrad, but support structure and services for the detectors will limit how much of the bore can be filled with active detector material. As designs progress, it may be possible to achieve a larger acceptance in the dipole spectrometer at both IP6 and IP8.

On the other hand, for lower-energy proton beams, unavoidable inefficiencies will occur in the transition regions. There is a low-$p_T$ cutoff due to the beam itself, which is most severe for the detection of recoil protons from mid- to high-energy beams (which provide the highest luminosity), for light ions at all energies, and for heavy ion fragments with A/Z close to that of the original beam. For ions, where the $p_T$ \textit{per nucleon} is usually small, acceptance at very low-$p_T$ is extremely important. With a traditional IR layout, low-$p_T$ acceptance can be improved by reducing the angular spread of the beam via reduced beam focusing. However, this has the drawback that it also reduces luminosity and still does not make it possible to reach $p_T$=0.
 

\begin{figure}[htb]
    \centering
    \includegraphics[width =0.9\textwidth]{figures/Unshifted_IP6_FF_Yellow_Report_flipped.pdf}
    \caption{Layout of the IP6 Far-Forward region generated with the EICROOT simulation package~\cite{EICroot} including the dipole magnets (rectangular boxes), quadrupole magnets (cylinders), and the four detector subsystems currently proposed to cover the geometric acceptance.}
    \label{fig:IP6_FF_layout}
\end{figure}

The kinematics of the EIC are uniquely suited to a more sophisticated forward detection concept than previous colliders. In DIS, the typical longitudinal momentum loss $dp/p \sim x$. At the same time, the intrinsic momentum spread of the particles in the beam is a few $\times 10^{-4}$. With a 10$\sigma$ margin, \textit{all} recoil protons with $x>0.01$ will thus separate out from the beam even at $p_T$=0, and at much lower $x$ for non-zero $p_T$. Since this method only relies on a fractional longitudinal momentum loss (magnetic rigidity), it is independent of the beam energy. For heavy ions, which typically only experience small changes in momentum, rigidity ($\sim A/Z$) can change through emission of nucleons. In particular, emission of a single neutron from an $A\sim100$ nucleus corresponds do a change in rigidity at the 1\% level, which in principle also allows the EIC to detect most nuclear fragments.

To take full advantage of the EIC kinematics, the forward detection requires two elements: dispersion and focusing. The former is generated by dipole magnets and translates a momentum (rigidity) change into a transverse position offset: $dr = D dp/p$ (\textit{e.g.}, with $D=40 cm$, the transverse displacement for a particle with $dp/p=0.01$ and $p_T=0$ will be 4 mm). This value has to be compared with the (10$\sigma$) beam size at the detection point (Roman pot). Without focusing, this is typically a few cm, but with a secondary focus it can be reduced to 2-3 mm (depending on the beam momentum spread). The beam size on the Roman pot does in principle not depend on the focusing of the beam at the collision point ($\beta^*$), but in a practical implementation the same magnets are used to generate both the primary and secondary focus. However, in contrast to the unfocused case, this means that with a secondary focus the best low-$p_T$ acceptance is achieved at the highest luminosity.
A secondary focus could in principle be used at either IP6 or IP8 of the EIC. However, while the current IP6 layout has some dispersion (17 cm), it does not have a secondary focus. In contrast, IP8 is  designed for a much larger dispersion and incorporates a secondary focus – making it complementary to IP6 and opening up unique physics capabilities, as can be seen in Fig.~\ref{fig:FF_layouts}.

\begin{figure}[htb]
    \centering
    \includegraphics[width =0.99\textwidth, trim={51mm 0mm 0mm 0mm}, clip]{figures/pt_vs_xL_comparison_plots.pdf}
    \caption{Two-dimensional plots of proton acceptance in transverse momentum, $p_{T}$ the nucleon momentum fraction. The acceptence is shown for three configurations: accepted protons in the IP6 Roman pots with the CDR high divergence optics (left), for accepted protons in the IP6 Roman pots with the CDR high acceptance optics (middle), and for accepted protons in the IP8 Roman pots at the secondary focus with the preconceptual optics configuration (right). All samples were generated for 18 GeV on 275 GeV protons with an $x_{L} > 0.8$ and with $0 < \theta < 5$ mrad; the cutoff at the top of the plots is due to the event generation region, while the acceptance in the bottom right varies with different configurations.}
%    \caption{Two-dimensional plots of transverse momentum, $p_{T}$ vs. the nucleon momentum fraction, $x_{L}$ for a generated proton sample (first pane), for accepted protons in the IP6 Roman pots with the CDR high divergence optics (second pane), for accepted protons in the IP6 Roman pots with the CDR high acceptance optics (third pane), and for accepted protons in the IP8 Roman pots at the secondary focus with the preconceptual optics configuration (fourth pane). All samples were generated with an $x_{L} > 0.8$ and with $0 < \theta < 5$ mrad. All of the optics configurations are for the 18x275 electron + proton beam energy configurations.}
    \label{fig:FF_layouts}
\end{figure}


\subsection{Detection of recoil baryons and light ions}\label{sec:ff:recoilions}

As discussed in sections 7.2.2 and 7.3.8 of the Yellow Report~\cite{AbdulKhalek:2021gbh} and earlier in this paper, exclusive reactions on the proton and light nuclei form an essential part of the EIC physics program. The wide kinematic reach of the EIC makes it ideal for probing different parts of the nuclear wave function, revealing how the internal landscape of nucleons and nuclei changes with $x$. Measurements of exclusive processes require high luminosity, a range of collision energies, and excellent far-forward detection. Key issues are detector acceptance for the recoil proton or light ion and optimized reconstruction resolution of the momentum transfer, $t$.

\paragraph{Proton detection:} Detecting the recoiling nucleons is important to cleanly establish the exclusivity of the reaction. It also makes it possible to reconstruct $t$ directly from the proton. Since the EIC reaches its highest luminosity with the most asymmetric beam energies (\textit{i.e.}, 5-10 GeV electrons colliding with hadrons at maximum energy), it is essential that the far-forward detection works optimally for high-energy protons. Here, the greatest challenge is to detect low-$p_T$ protons which stay within the beam envelope. This capability can be improved by using a secondary focus, which essentially provides full acceptance for $x>10^{-2}$, and significantly improves the low-$p_T$ acceptance for lower $x$. For lower proton beam energies, a secondary focus is still useful, although less crucial. However, at lower energies, high-$p_T$ protons will start experiencing losses in the apertures of the accelerator quadrupole magnets, leading to a reduced acceptance for detectors downstream of these magnets. Embedding a tracking detector, such as is envisioned with the B0 tracker in IP6, provides increased coverage of high-$p_{T}$ protons at the lower beam energies. This issue can be alleviated by using magnet technologies that allow for higher peak fields, which makes it possible to increase the apertures, but there are other technical constraints that could make this challenging, especially at IP6, and more study is needed to determine what level of improvement is possible. In conjunction with a secondary focus, this would further enhance the capabilities of the EIC to do transverse proton imaging.

\paragraph{Determination of $p_T$ in exclusive reactions:} Another important consideration for exclusive reactions is reconstruction of $t$. In principle it can be done either by using the recoiling system detected in the far-forward detectors, or from the scattered electron and produced particle (charged meson or DVCS photon) detected in the central detector. There are advantages to both methods. For example, the former method is very straightforward, but requires a good understanding of the beam effects (e.g. angular divergence). Ideally one would want to be able to apply both, but this requires that the central detector can provide a sufficiently good $p_T$-resolution. This is a challenge for a tracker, but even more so for the EM calorimetry if one wants to be able to determine $t$ ($\Delta_\perp$) from the DVCS photon (or the photons from $\pi^0$ production). However, while such a dual capability is useful for protons, it becomes essential for ions, where the ability to determine $t$ from the ion is more limited and vanishes entirely when the ion is not detected (high A and low $p_T$). Being able to determine $t$ from the DVCS photon would thus greatly enhance the ability to do transverse imaging of ions.

\paragraph{Light ion detection:} Coherent exclusive scattering on light ions differs from protons in two ways. First, the available ion beam energies are restricted a range between 100 GeV/A and $275 \times Z/A$ GeV/A, as well as a discrete energy at 41 GeV/A. Second, scattered ions travel much closer to the beam, making low-$p_T$ acceptance very challenging (and conversely, the high-$p_T$ acceptance much less so, even for the high-$t$ tails). This is the combined result of two effects: cross sections for ions peak at lower $t$, and a given $t$ corresponds to a lower $p_T$ per nucleon. The former means that in contrast to the proton, clean imaging of light ions \textit{requires} an acceptance down to $p_T \sim 0$, and the latter that implementing such an acceptance is particularly difficult. A secondary focus is thus essential for high-quality measurements of coherent scattering on light ions.
However, if the central detector has the ability to reconstruct the $p_T$ from the produced photon or meson as discussed above, a secondary focus would allow for a hybrid method where ions with higher $p_T$ are detected (the incoherent backgrounds become more challenging as one moves towards the first diffraction minimum), while the low-$p_T$ part is reconstructed by vetoing the breakup (which is generally easier to do with light than heavy ions). A hybrid measurement would not be as clean as one where all recoiling ions are detected, but it would make it possible to reach lower $x$ and higher A, extending the discovery potential of the EIC.

\subsection{Spectator detection}

Detection of nuclear breakup is essential for a broad range of EIC physics topics. From a detection perspective, these broadly fall into two categories: spectator nucleons and nuclear fragments.
In the first case, the spectator nucleon typically experiences a very small change in momentum, but its magnetic rigidity (A/Z) is very different from that of the original beam. A proton spectator will thus initially continue moving with the beam, but will separate quickly from it after passing the first dipole magnet. The detection challenge here thus lies primarily in providing adequate magnet apertures.
%When comparing to the case when we detect the recoiling system, the detection challenge is similar to that for high-$p_T$ protons, and as such is not directly related to a secondary (although it could be more broadly to the use of more advanced magnet technologies in IR8).
An key example of spectator proton tagging are measurements of neutron structure in deuterium and $^3He$. 

In the case of nuclear fragments, they may be detected as a way of vetoing breakup or part of the direct measurement. 
The former case was discussed above (Sec.~\ref{sec:ff:recoilions} in the context of light and medium nuclei, but coherent processes on heavy ions are different in that even with a secondary focus, the high-$p_T$ tails cannot be measured directly as the ion always stays inside the beam envelope. A secondary focus can, however, make it possible to detect residual ions that have lost a single nucleon (A-1 tagging). Adding such a capability will significantly improve the efficiency for vetoing the large incoherent backgrounds, making a reasonably clean measurement possible. 

Finally, there are several measurements that rely on detection of the spectator nucleons, the residual nucleus, or nuclear fragments in the final state. One example is the case when the struck nucleon and its partner are in a short-range correlation with a high relative momentum. In this case, the spectator nucleon will not only have a different A/Z compared with the original ion, but also a large $p_T$. The breakup kinematics can then be best constrained if the residual A-2 nucleus can be detected, which is facilitated by a forward spectrometer with a secondary focus. A related topic is detection of rare isotopes produced in the interaction, which is discussed in Sec.~\ref{sec:ff:isotopes}. Additional detail, including discussion of the theoretical framework for several of the tagged measurements can be found in Ref.~\cite{Strikman:2017koc, Cosyn:2020kwu}

%At the EIC, e-A scattering also produces rare isotopes. Here, relativistic kinematics are particularly useful for measuring the photons from excited states, which can be measured in coincidence with the rare isotope. The improved acceptance from a secondary focus greatly increases the amount of isotopes that can be studied, creating a potential for a program that would be complementary to the one at FRIB.

\paragraph{Neutron structure through spectator tagging}

Light ion beams can be used as an effective free neutron target via spectator tagging. Deuterium is the simplest system, while $^3He$ can be polarized (70\%) and thus give access to the neutron spin structure. Spectator tagging can be applied to any primary measurement ($F_2$, DVCS, etc), but a key common challenge is to account for final-state interactions (FSI). However, recent studies~\cite{Jentsch:2021qdp} have shown that free neutron structure can be extracted by on-shell extrapolation to the non-physical pole, where the neutron is by definition free and unaffected by FSI. In contrast to the pion, this approach is much more robust for the heavier nucleon where the extrapolation takes place over a shorter interval. The extrapolation is done by fitting the measured $t$ distribution, but focuses on the low-to-modest values of $t$ part, where the extrapolation has minimal model dependence.

Experimentally, this measurement relies on a high-resolution determination of the $p_T$ distribution, and of having sufficiently large magnet apertures to tag a spectator proton with low $p_T$~\cite{Jentsch:2021qdp}.
As a cross check, it is also possible to apply the same method to the bound proton by tagging the neutron from deuterium in the ZDC.

%%%%%%%%%%%%%%%%%%%%%%%% PNT

\paragraph{Proton and neutron spectators from deuteron beams}


Deuteron beams can be used as an effective free neutron target via spectator tagging, where the undisturbed proton is measured to isolate scattering from the proton. To isolate nearly on-shell neutrons, the goal is to tag protons which had low initial momenta (corresponding to low $-t$) in the deuteron rest frame. Measurements will be made over a range of $t$, so that the extrapolation to the on-shell neutron can be performed over different ranges of $t$ to ensure stability of the extrapolation. As noted above, detection of these protons in the Off-Momentum Detector and Roman Pots is relatively straightforward and the key issue is minimizing the loss of acceptance in the apertures of the accelerator magnets. 





Similar studies of the proton structure of the proton structure can be performed with neutron tagging used to isolate scattering from a low-momentum proton. In this case, the results can be compared to the known proton structure, and these studies can be used to study the $t$-dependence and test the extrapolation to the on-shell proton. For the low $t$ values required for these measurements, the neutrons have $x_L$ near unity and small $P_T$ and are detected in the ZDC.


%\paragraph{Tagged proton structure - neutron spectators from deuteron beams}


\paragraph{Double tagging from 3He breakup}

While the deuteron is the most common target used to study unpolarized neutron structure, polarized $^3$He serves as the most effective target for measuring neutron spin structure, as the neutron carries most of the spin in $^3$He. Inclusive measurements can provide some information, with the protons acting mainly as a dilution to the asymmetries associated with scattering from the polarized neutron. But double tagging of the two spectator protons in $^3$He can be used to isolate scattering from the neutron without dilution or corrections for the proton contributions~\cite{Friscic:2021oti}. In this case, the goal is to measure spectators with low momenta in the $^3$He rest frame which have momenta close to the beam momentum per nucleon and small $P_T$, but lower mass and therefore roughly 2/3 of the rigidity of the $^3$He beam. One can also examine events with one large-momentum proton to identify high-momentum neutrons in the initial state to look at the spin structure as a function of initial neutron momentum, which is relevant for understanding the spin EMC effect. 


\paragraph {Tagged Pion structure - nucleon spectators from proton beams}
%{\em Draft text by Garth Huber, Oct 10}

Measurement of the $\pi^+$ electromagnetic form factor can be accomplished at the EIC by the detection of the neutron spectator in coincidence with the scattered electron and $\pi^+$, i.e. an exclusive reaction with $e'-\pi^+-n$ triple coincidence. The neutron is emitted with 80-98\% of the proton beam momentum, and is detected in the ZDC.  The pion form factor measurement only requires $-t$ measurements up to about 0.4~GeV$^2$, so a moderate acceptance ZDC is sufficient to catch the events of interest.  Very good ZDC angular resolution is required for two reasons. First, to separate the small exclusive $\pi^+$ cross section from dominant inclusive backgrounds, a cut may be placed on the detected neutron angle in comparison to the reconstructed neutron angle (from $e'$ and $\pi^+$ using momentum conservation). Second, a $t$ reconstruction resolution better than $\sim$0.02~GeV$^2$ is necessary for a quality form factor measurement and such resolution is only possible when reconstructed from the initial proton and final neutron momenta.  The ZDC is thus of crucial importance to the feasibility of a pion form factor measurement at the EIC.

\paragraph{Tagged Kaon structure - hyperon spectators from proton beam}
%{\em Draft text by Garth Huber, Oct 11}

Measurements of the $K^+$ electromagnetic form factor at high $Q^2$ via the Sullivan process would yield valuable information on nonperturbative DCSB--Higgs-boson interference effects in hard exclusive processes.  
The reaction of interest is $e + p \rightarrow e'+K^+ +\Lambda$, where the $\Lambda$ is emitted with $>70$\% of the proton beam momentum.  We expect that lower beam energies are optimal, to ensure a high $\Lambda$ decay fraction, as non-decayed $\Lambda$ will be impossible to distinguish from neutron hits.

The $\Lambda$ needs to be identified from its decay products to ensure the clean identification of the exclusive events from inclusive backgrounds, and to reconstruct $t=(p_p-p_{\Lambda})^2$ with sufficiently high resolution.  One complication is that the $\pi^-$ from the dominant $\Lambda\rightarrow p\pi^-$ decay channel cannot be detected in the far forward detectors for decays occurring at or after the B0 magnet. Such measurements would require dedicated detectors for negative particles or be limited to decays occurring sufficiently before B0.  The neutral $\Lambda\rightarrow n\pi^0\rightarrow n\gamma\gamma$ decay seems a better choice.  For the measurement to be feasible, three hit events need to be reliably identified in the ZDC with sufficiently good energy and angle resolution for $t$ reconstruction.  Even more challenging is confirming that the Sullivan process dominates at low  $-t$, which requires a measurement of the $\Lambda/\Sigma^0$ ratio. This entails the reliable detection of four neutral hits in the ZDC, from $\Sigma^0\rightarrow\Lambda\gamma\rightarrow n\pi^0\gamma$. Thus, this is a measurement that is significantly more challenging than that of the pion form factor, although if it is feasible, it would be an important addition to the EIC scientific program. The acceptance for neutral decay products could potentially be increased significantly if calorimetry were included in the B0 magnet. This option was mentioned as a possibility in the Yellow Report, but including both tracking and calorimetry is technically challenging due to spatial constraints inside the magnet and further design work is needed to know what is be possible.




\subsection{Tagging of active nucleons - high spectator momenta}

%{\em Draft text by Alexander Jentsch}

While the previous sections focused on tagging of relatively low-momentum spectators, other key studies are focused on isolating high-momentum nucleons and/or mapping out tagged nucleon structure over a wide range of initial virtualities.
Studies of Short-Range Correlations between pairs of bound nucleons require tagging of final state nucleons at both high and low values of $p_T$ to fully exploit the measurement capability. This provides a unique challenge for the detector acceptances, as multiple far-forward subsystems play a role in covering the phase space. In general, the active nucleon in a reaction will be scattered with relatively large polar angles ($\theta > 5 mrad$), while the recoil nucleons and spectator nuclear fragments (for A $>$ 2) are usually at smaller values. Additionally, in the case of the recoil protons, there is a magnetic rigidity change with respect to the ion beam which further complicates detection. It is in principle also possible to tag an A-2 spectator nucleus, in the final state, but this is uniquely challenging to do the small scattering angles for the spectator nucleus, and the small rigidity change, dependent on the struck SRC pair. Tagging of A-2 nuclei can be enhanced with Roman Pots at a secondary focus.

In cases where both final-state nucleons from an SRC pair are measured, the spectator nucleon is detected in the far-forward region while the active (struck) nucleon is measured in the main or far-forward detectors. At higher energies, the acceptance is more complete when measuring a spectator neutron and active proton, since the polar angle coverage for struck protons is extended to $\sim20$mrad in the B0 tracking detector, while the neutron acceptance is limited to $\sim5$mrad by the magnet aperture. For active neutrons, the lower beam energy configurations (e.g. 5x41 GeV/n) are more beneficial since the larger active neutron scattering angle can place them in the acceptance of the main detector endcap hadronic calorimeter (i.e. $\theta > \approx30$~mrad). Additionally, if more of the open bore space in the dipole spectrometer can be used for active detector material, it would further enhance the capabilities for active proton tagging beyond the current 20 mrad assumption.

Having some capability for tagging in the higher-$p_T$ regime allows simultaneous study of both free nucleon structure and nuclear modifications with the same experimental setup. Studies of Short-Range Correlations and nuclear modifications enable the EIC to provide insight into the EMC effect and other physics at higher-x.

\subsection{Vetoing of breakup}

%{\em Draft text by Spencer Klein, started Oct. 12}

Separation of coherent and incoherent photoproduction of photons (Deeply Virtual Compton Scattering) and vector mesons is critical to many aspects of the EIC physics program.  In the Good-Walker paradigm, one can relate the coherent cross-section to the average nuclear configuration, while the incoherent cross-section is sensitive to event-by-event fluctuations of the nuclear configuration, including gluonic hot-spots~\cite{Klein:2019qfb}.  One can do a two-dimensional Fourier transform of $d\sigma_{\rm coherent}/dt$ to determine the transverse distribution of gluons in the nuclear target - the nuclear equivalent of the GPD.  By studying different mesons with different masses, and using photons with different $Q^2$, one can map out nuclear shadowing as a function of position within the nucleus.   

The challenge in these measurements is in adequately separating coherent and incoherent production, by detecting the products of nuclear breakup~\cite{Chang:2021jnu}. To determine the transverse gluon distributions, it is necessary to measure $d\sigma_{\rm coherent}/dt$ out to the third diffractive minimum~\cite{AbdulKhalek:2021gbh}, to avoid windowing artifacts in the Fourier transform.  At this minimum, a rejection factor of 500:1 is needed to adequately remove the incoherent background.   

In most cases, nuclear dissociation leads to neutron (or, less frequently, proton) emission from the target. These are relatively straightforward to detect, although very high efficiency is required. However, some soft excitations will produce excited nuclear states that decay by photon emission.  These photons typically have energies of a few MeV (or less) in the nuclear rest frame.  Gold (planned as the main EIC heavy nuclear target), is particularly bad.  It has a 77 keV excited state with a 1.9 nsec lifetime.  Because of the lifetime, this state is almost impossible to observe in an EIC detector.  It's next states have energies of 269 and 279 keV respectively.  The lab-frame energies depend on the EIC beam energies, but for 110 GeV/n gold beams, the maximum energy is 65 MeV.  For photon emission away from the far-forward direction, the energy will be lower.  This is likely beyond the reach of the planned EIC detectors, but could be accessible in an upgrade. Because the energy transfer to the target (and hence the energy spectrum of the excitations) depends on $t$, is it critical to be able to detect emission of protons, neutrons, and soft photons over the full phase space. As noted earlier, the addition of calorimetry in the B0 magnet would improve the acceptance, but is technically challenging.

Since the knockout of a single neutron (and possibly evaporation of another) is an important contribution to the incoherent background, the ability to tag and veto on A-1 nuclei (\textit{e.g.}, Zr-89 from a Zr-90 beam) is also very important for a clean measurement. High-resolution photon detection is also synergistic with a potential rare isotopes program discussed below.

It is also possible to mistake coherent production for incoherent, if a second collision in the same beam crossing dissociates a nucleus~\cite{Klein:2014xoa}.  This could affect the measurement of the incoherent cross-section at small $|t|$.  Although the background rate can be subtracted, statistical uncertainties will remain.  However, most of these events can be removed if the ZDC has very good timing.



\subsection{Backward (u-channel) photoproduction}

%{\em Draft text by Spencer Klein, started Oct. 13}

In backward (u-channel) photoproduction, the produced meson takes most of the energy of the incident proton, and so goes in the forward direction, while the proton is shifted many units of rapidity, and, at the EIC, is visible in the central detector~\cite{Gayoso:2021rzj}.  Instead of having small Mandelstam $t$, as in conventional photoproduction, $t$ is large (near the kinematic maximum) and $u$ is small. This process may be modelled using Regge trajectories involving baryons, but it is not easy to see how such simple reactions can lead to nucleons being shifted many units of rapidity; there may be connections with baryon stopping in heavy-ion collisions.   A systematic exploration of production of different mesons at higher energies is needed to fully characterize this reaction, and test the Regge trajectory approach. 

Reconstruction of these events requires a forward detector that is able to reconstruct multi-particle final states.  For the full 18 $\times$ 275 GeV beam energy, the products of light meson ($\omega$, $\rho$ or $\pi^0$) mostly end up with $\eta >6.2$, in the zero degree calorimeter (ZDC).  At lower beam energies, or with heavier mesons, the products at are at smaller pseudorapidity. This requires a forward detector with as full an acceptance as possible ({\it i. e.} with no holes in acceptance) for both charged and neutral particles.


\subsection{Rare isotopes (including photons for spectroscopy)}\label{sec:ff:isotopes}

%{\em Draft text by Barak Schmookler}

As discussed in the recent EIC Yellow Report, simulation studies suggest that the EIC has the potential to produce and detect rare isotopes along with their gamma photon decays, allowing this new machine to complement the results from dedicated rare isotope facilities.

Direct detection of the rare isotopes will use the Roman Pot (RP) detectors. At first approximation, the produced rare isotopes will have the same momentum-per-nucleon as the ion beam and no angle relative to the beam. Under this approximation, the rigidity (R = p/Z) of the isotope is directly related to its A/Z as
%
\begin{equation}
R_{Rel} = (R - R_{beam})/R = \Delta p / p = \left(\frac{A}{Z}\right) / \left(\frac{A_{beam}}{Z_{beam}}\right) ~.
\end{equation}
%
Under the above assumption, the isotope's hit position in the dispersive direction at the RP gives a measurement of A/Z. Figure~\ref{fig:rigidity_isotopes} shows the expected hit positions for known and predicted isotopes both at the first RP for the primary IR and at the first RP located near the secondary focus in the second IR, assuming a $^{238}$U beam. Isotopes with the same Z and different A values are shown at the same vertical position in the plots. In addition, using the beam parameters from table~3.5 of the 2021 EIC CDR~\cite{} for heavy nuclei at 110 GeV/A on electrons at 18 GeV, the 10$\sigma$ beam exclusion are is shown by the gray box. As can be clearly seen, none of the heavy rare isotopes can be detected in the primary IR, while the second IR has the potential to detected the majority of the isotopes.  At the RP in the second IR, isotopes with the same Z that differ by a single neutron are expected to be separated by 1.5 mm for Z = 100 and 5 mm for Z = 25.

\begin{figure}[htb]	
        \includegraphics[keepaspectratio=true,width=3.4in,page=1]{figures/IR6_RP1.pdf}		
		\includegraphics[keepaspectratio=true,width=3.4in,page=1]{figures/IR8_RP1.pdf}
	\caption{Left: Isotope Z vs. hit position in the first RP for the primary IR; right: Isotope Z vs. hit position in the first RP at the secondary focus for the second IR. The gray box on each plot shows the 10$\sigma$ beam exclusion area. The plots are made assuming a $^{238}$U beam.}
	\label{fig:rigidity_isotopes}
\end{figure}

For uniquely determining the isotope, a direct measurement of Z is needed. The simplest way to do this is by placing a Cherenkov detector behind the RPs at the secondary focus. The number of Cherenkov photons produced by the isotope will be proportional to Z$^2$.

Measuring gamma decay photons is also important as the level transitions reveal the structure of the final isotope. The photons are produced isotropically in the isotope's rest frame but can be Lorentz up-shifted significantly in the lab frame. This shift, as well as the requirement that these photons be detected in coincidence with an isotope, means that photon background will be small. LYSO crystals that do not require cryogenics can therefore be used for this measurement. In addition, while spectroscopy would benefit from a good photon acceptance, it would not be a critical requirement.
